A Comparative Study of Compressive Sensing Algorithms for Hyperspectral Imaging Reconstruction

Hyperspectral Imaging comprises excessive data consequently leading to significant challenges for data processing, storage and transmission. Compressive Sensing has been used in the field of Hyperspectral Imaging as a technique to compress the large amount of data. This work addresses the recovery of hyperspectral images 2.5x compressed. A comparative study in terms of the accuracy and the performance of the convex FISTA/ADMM in addition to the greedy gOMP/BIHT/CoSaMP recovery algorithms is presented. The results indicate that the algorithms recover successfully the compressed data, yet the gOMP algorithm achieves superior accuracy and faster recovery in comparison to the other algorithms at the expense of high dependence on unknown sparsity level of the data to recover.

==> 2.4-CD_algorithm.tex <==













\subsubsection{CD Algorithm}
Let us note that $g(\xb)$ in problem (\ref{eq:optPb}) is separable and thus we can apply a scheme based on a coordinate-wise update rule such as coordinate descent. The advantage of this approach lays in the fact that the cost per iteration is of order $O(N)$ since we only have operation with vectors. The convergence rate of this method is $O(1/k)$\cite{necoara2016parallel}.

\begin{algorithm}
	\caption{ CD}
	\begin{algorithmic}
		\STATE \textbf{Input:} Starting point $\xb_0 \in \mathbb{R}^N $, $\lambda$, level of tolerance $\epsilon$.\\
		\STATE \textbf{Initialization:} $\Delta$ =1, k=1
		\STATE \textbf{Compute} for all $i \in \left[1,N\right]$ Lipschitz constants $L_i = \| \mathbf{a}_i \|^2$.
		\STATE Compute initial residue $\rb = \Ab \xb_{0} - \yb$
		\WHILE{\Delta > \epsilon}{
			\STATE 1. Choose uniformly random an index $i \in \left[1,N\right]$.
			\STATE 2. $\text{aux} \gets \xb^i_{k-1} - \frac{1}{L_i} \mathbf{r}^T\mathbf{a}_i$
			\STATE 3. $\xb_{k}^{i} \gets \text{sign(aux)$ \cdot$ max}(|\text{aux}| - \frac{\lambda}{L_i},0)$
			\STATE 4. $\rb \gets \rb+(\xb_{k}^i - \xb_{k-1}^i)\mathbf{a}_i$
			\STATE $\quad\Delta \gets \| \xb_{k} - \xb_{k-1}\|_2$,  $\quad k \gets k+1$}
	\end{algorithmic}
	\label{alg:cd}
\end{algorithm}






